A Combined First Principles Study of the Structural, Magnetic, and Phonon Properties of Monolayer CrI$_{3}$

The first magnetic 2D material discovered, monolayer (ML) CrI$_3$, is particularly fascinating due to its ground state ferromagnetism. Yet, because monolayer materials are difficult to probe experimentally, much remains unresolved about ML CrI$_{3}$'s structural, electronic, and magnetic properties. Here, we leverage Density Functional Theory (DFT) and high-accuracy Diffusion Monte Carlo (DMC) simulations to predict lattice parameters, magnetic moments, and spin-phonon and spin-lattice coupling of ML CrI$_{3}$. We exploit a recently developed surrogate Hessian DMC line search technique to determine CrI$_{3}$'s monolayer geometry with DMC accuracy, yielding lattice parameters in good agreement with recently-published STM measurements - an accomplishment given the $\sim 10$% variability in previous DFT-derived estimates depending upon the functional. Strikingly, we find previous DFT predictions of ML CrI$_3$'s magnetic spin moments are correct on average across a unit cell, but miss critical local spatial fluctuations in the spin density revealed by more accurate DMC. DMC predicts magnetic moments in ML CrI$_3$ are 3.62 $\mu_B$ per chromium and -0.145 $\mu_B$ per iodine; both larger than previous DFT predictions. The large disparate moments together with the large spin-orbit coupling of CrI$_3$'s I-$\textit{p}$ orbital suggests a ligand superexchange-dominated magnetic anisotropy in ML CrI$_3$, corroborating recent observations of magnons in its 2D limit. We also find ML CrI$_3$ exhibits a substantial spin-phonon coupling of $\sim$3.32 cm$^{-1}$. Our work thus establishes many of ML CrI$_{3}$'s key properties, while also continuing to demonstrate the pivotal role DMC can assume in the study of magnetic and other 2D materials.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> xx.tex <==


